A review and experimental evaluation of deep learning methods for MRI reconstruction

Following the success of deep learning in a wide range of applications, neural network-based machine-learning techniques have received significant interest for accelerating magnetic resonance imaging (MRI) acquisition and reconstruction strategies. A number of ideas inspired by deep learning techniques for computer vision and image processing have been successfully applied to nonlinear image reconstruction in the spirit of compressed sensing for accelerated MRI. Given the rapidly growing nature of the field, it is imperative to consolidate and summarize the large number of deep learning methods that have been reported in the literature, to obtain a better understanding of the field in general. This article provides an overview of the recent developments in neural-network based approaches that have been proposed specifically for improving parallel imaging. A general background and introduction to parallel MRI is also given from a classical view of k-space based reconstruction methods. Image domain based techniques that introduce improved regularizers are covered along with k-space based methods which focus on better interpolation strategies using neural networks. While the field is rapidly evolving with plenty of papers published each year, in this review, we attempt to cover broad categories of methods that have shown good performance on publicly available data sets. Limitations and open problems are also discussed and recent efforts for producing open data sets and benchmarks for the community are examined.

==> sections/rebuttal.tex <==
\begin{center}
    {\large \textbf{Legends that we have used in this rebuttal}}
\end{center}
1. First reviewer: \ra\\
2. Second reviewer: \rb\\
3. Third reviewer: \rc\\
4. Our Response: [\textcolor{blue}{Response}]\\
5. Questions are in \textit{italic}\\
6. Website/code are in \texttt{typeset}\\
7. Citations are marked as [\textcolor{red}{number}]\\
8. Any text modification in the main draft\colorbox{blue!05}{ is highlighted using this color}\\
\textbf{\underline{We request all reviewers to see BOTH:}}\\
Response to \textbf{common questions/suggestions}, and\\
Response to \textbf{Reviewer X}, where X is the reviewer number.\\
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%
%%%
%

\noindent We thank the reviewers and the handling editor for their helpful comments and suggestions. 
We are encouraged that they found the draft is well categorized (\ra, \rb), the survey paper can be a valuable review article (\ra, \rb, \rc),  and the theoretical basics and experimental comparison of a selection of methods on an open-source dataset would help the community (\ra). 
We are pleased that \rb\ recognizes our mention of the limitations of deep learning models such as generalization, robustness, and data efficiency. 
We are glad to note that the \ra\ has found that our paper has a broader scope and \rc\ appreciated the Generative Network based MRI reconstruction section, i.e. Sec. \ref{sec_generative_model}. 
There are a few comments and concerns raised by \ra, \rb, \rc, which we address below and in the manuscript.
We have used \textcolor{blue}{blue color to denote} any modification or change of the draft. 
Below, we give point-wise response to all questions and comments.\\
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%
%%%
%
\noindent \dotfill
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%
%%%
%
\begin{center}
    {\large \textbf{Recap of our work}}
\end{center}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
\noindent\textbf{What is our goal?} To consolidate and summarize generative and non-generative deep learning methods for accelerated MRI reconstruction along with a general background and introduction of classical k-space based reconstruction methods. 
We experimentally compared a selection of methods on an open source dataset. 
We discussed different challenges such as robustness, risk quantification, generalization, etc., of deploying deep neural networks for accelerated MRI reconstruction.\\
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
\noindent\textbf{Why this goal?} To help researchers get a holistic view of the field that spans the classical methods, deep learning generative methods, and deep learning non-generative methods. 
At the same time making them aware of the limitations and open problems of deep learning based accelerated MRI reconstruction methods.\\
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%%%
%%%
%
\newpage
\begin{center}
    {\large \textbf{Responses to the common questions/suggestions}}
\end{center}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{Merge Bayesian Learning, VAE, and PixelCNN+}: \\
\ra\ \textit{Sections 4.2 & 4.3 should be merged in one section on Bayesian learning with a slightly broader and expanded scope. E.g.: “From a Bayesian perspective, we can improve upon ML through maximum a posteriori (MAP) estimation. The framework of variational autoencoders (VAEs) provides a computationally efficient way for optimizing Deep Latent Variable Models jointly with a corresponding inference model using SGD.”} [Kingma and Welling, 2019]\\
\rb\ \textit{Section 4.2 and 4.3. Using VAEs (4.2) to estimate prior is one case of Bayesian learning (4.3). To be coherent, I suggest the authors combine 4.2 and 4.3 together as the Bayesian learning section, list VAE, and PixelCNN+ for prior estimation.}\\
%%%%%%%%%%%%%%%%%%%%%
\response Thank you for the comment. 
We have updated the paper and merged the two sections. 
Now, Sec. 4.2 "Bayesian Learning" provides a study of Monte Carlo estimation, Variational Autoencoder (VAE), PixelCNN+. 
In addition to this, we added one more discussion of Recurrent Inference Machine (RIM) [Lønning, K. et al. (2019)]. 
Thank you for pointing out the RIM paper that we initially missed.\\
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{Dynamic or Temporal Data}:\\
\ra: \textit{Is dynamic/temporal data disregarded altogether?}\\
\rb: \textit{\dots it would be better to extend the review a little to k-t space recon, and review some of the classical methods (e.g., k-t SENSE, k-t GRAPPA, k-t FOCUS, etc) and deep learning ones (e.g., CRNN).}\\
\response We have added dynamic MRI references in the main draft based on the context. 
For example: the \citep{huang2005k, lustig2006kt, otazo2015low} etc. methods come under the classical dynamic MRI reconstruction algorithms (see Sec. 1.3.), and Variational approach \citep{rasch2018dynamic} (in Sec. 2.2.). 
While, methods such as \citep{biswas2019dynamic, schlemper2017deep, seegoolam2019exploiting} (see Sec. 5.3. Inverse Mapping for Image Rectification), CRNN \citep{qin2018convolutional} (see Sec. 5.4.), Deep Image Prior based dynamic MRI model \citep{yoo2021time} (see Sec. 5.2.), etc., methods come under Deep Learning based dynamic MRI reconstruction methods. 
We agree with \rb\ that the primary focus of this survey is to consolidate and summarize generative and non-generative deep learning methods for accelerated MRI reconstruction along with a general background and introduction of classical k-space based reconstruction.\\
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{The dimension is 2D/3D?} \\
\ra: \textit{Line 47,66: the introduction of dimensions is inconsistent (2D/3D).}\\
\rc: \textit{3D is a volume. Also I want to add that 4D and 5D applications exist where additional indices show up.}\\
\response Thank you for the suggestion! We have changed the sentence.\\

\noindent [\textbf{Please Turn Over}\dots]
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
\newpage
\begin{center}
    {\large \textbf{Response to \ra}}
\end{center}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Paper tile}: \textit{The title of the manuscript (‘review’) refers to a conventional literature review paper. This work has a broader scope.}\\
%%%%%%%%%%%%%%%%%%%%%
\response Thank you for the suggestion! We have changed the title to - ``A review and experimental evaluation of deep learning methods for MRI reconstruction''.\\
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{Compare methods using fastMRI leaderboard:} \textit{A challenge is a common way to compare methods. Can the authors submit their outcomes to the fastMRI leaderboard and compare the scores to others?}\\
%%%%%%%%%%%%%%%%%%%%%
\response Excellent suggestion! We note that few algorithms, like Variational Net, GAN, Zero Filled are already in the fastMRI leaderboard. For others, we directly used the source code provided by the authors on GitHub. Since these methods are not our original developments and neither we modified any part of the source code, we are not entirely sure whether we are eligible to submit such third-party contents on the fastMRI leaderboard.  As such, we will communicate with the fastMRI challenge organizers and the authors of these source codes about such a possibility.\\
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{SSIM score:}\textit{How do they relate their highest SSIM-score to currently leading methods on the leaderboard?}\\
%%%%%%%%%%%%%%%%%%%%%
\response Please note that, we did not use images with a width greater than 372. We note that such data is only 7\% of the training data split. 
As a consequence the SSIM scores are sslightly lower with respect to their original scores as reported in the papers. 
We estimated the SSIM score using the following scikit software package;\\
\texttt{from skimage.measure import compare\_ssim}.\\
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{Table 1 score difference:} \textit{Line 868: the metrics reported for the VN in Table 1 for the VariationNET (Sriram et al., 2020a) deviate a lot from what’s reported in the paper. Although, on line 867 I read “We did not use images with a width greater than 372 and we note that such data is only 7\% of the training data split. Both the 4x and 8x acceleration factors were evaluated”.}\\
%%%%%%%%%%%%%%%%%%%%%
\response Indeed! The differences in the results can be explained due to the differences in the training dataset (7\% less training in our case).\\
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{VariationalNET:} \textit{Line 217: The VariationNET (Sriram et al., 2020a) is a follow-up work of Hammernik, K. et al. (2018). The PyramidRNN mentioned on line 822 is not.}\\
%%%%%%%%%%%%%%%%%%%%%
\response Here is a confusion! 
The VariationNET unrolls an iterative algorithm involving a CRNN based recurrent neural network based regularizer. 
We tried to show that the VariationNET followed the legacy of Convolutional Recurrent Neural Networks or CRNN (Qin et al., 2018) and the PyramidRNN. But, we agree to the point of \ra\ and added few lines in Sec. \ref{sec_nongen_rnn} to clarify its relation with both the work of Hammernik, K. et al.  (2018) and CRNN. 
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%
%%%%%%
%%
%
\newpage
\begin{center}
    {\large \textbf{Response to \rb}}
\end{center}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.1cm}

\noindent\textbf{Difference between spatial and temporal nets} \textit{Section 5.3 and 5.4. It is confused what is the major difference between spatial and temporal nets? For instance, DCCNN and ISTA nets in section 5.3 and IHT and CRNN nets in section 5.4 are all unrolled networks, but they were split into two categories.}\\
%%%%%%%%%%%%%%%%%%%%%
\response By \underline{spatial network}, we mean networks that unroll an iterative algorithm involving a receptive field based convolutional regularizer. 
Such receptive field based convolutional regularizer automatically and adaptively learn spatial hierarchies of features through backpropagation [\textcolor{red}{1}, \textcolor{red}{2}], for example: Convolutional Neural Networks and Transformer Networks. The \underline{temporal nets}, on the other hand, exhibits temporal dynamic behaviour using connections between nodes form a directed or undirected graph along a temporal sequence [\textcolor{red}{3}], for example: LSTMs, Convolutional Recurrent Neural Network (CRNN). 

Following these definitions, the ISTA-Net and the DCCNN are categorized under ``spatial network''. 
On the other hand, the ITH, the CRNN and its follow-up work VariationalNET are categorized under ``temporal network''. 

For the sake of simplicity, we have now renamed Sections \ref{sec_nongen_cnn} and \ref{sec_nongen_rnn} as\\ \colorbox{blue!05}{Convolutional Neural Networks} and \colorbox{blue!05}{Recurrrent Neural Networks}.
%%%%%%%%%%%%%%%%%%%%%s
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{More references on the topic of robustness} \textit{The authors discussed the stability/robustness of deep learning models in discussion. It would be more comprehensive if the authors can search for literatures to see what efforts have been done to improve the robustness of deep network models? For instance, in FINE [\textcolor{red}{6}], the pre-trained recon network was fine-tuned using data consistency to reduce generalization error inside unseen pathologies.}\\
\response Thank you for sharing this thought! 
We have rewritten Sec. \ref{sec_discussion} second paragraph to accommodate the discussion of robustness in terms of adversarial attack, i.e.;\\
%\colorbox{blue!05}{In this discourse the robustness of a DL based MR reconstruction method is also studied}\\
%\colorbox{blue!05}{in various papers $\dots$}\\
As per the suggestion, we have added few more references such as [\textcolor{red}{5}], FINE [\textcolor{red}{6}] and [\textcolor{red}{7}]. 

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Add MoDL [\textcolor{red}{4}] reference} \textit{Following comment 2, MoDL is another important unrolled deep reconstruction. It should be mentioned in the context}\\
%%%%%%%%%%%%%%%%%%%%%
\response Though we have added a recent development of MoDL that is called J-MoDL, we missed to add this. A description shown below and a citation are added to the modified draft, see the Sec. \ref{sec_nongen_cnn}
%), i.e.:\\
%\colorbox{blue!05}{Later, MODL \citep{MODL} proposed a model based MRI reconstruction}\\
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
\newpage
\begin{center}
    {\large \textbf{Response to \rc}}
\end{center}
%%%%%%%%%%%%%%%%
%%%%%%%%%%%
%%%%%%%
%%%
%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 1.1. Equation 3} \textit{\dots Because you introduced the coil sensitivity map before this seems incorrect. 
It could e.g. be fixed by saying $y_i$}\\
\response Thank you for pointing this out and giving the suggestion! 
We follow the formulation that appeared in \citep{sriram2020end, zheng2019cascaded}, i.e.;
\begin{equation}
\begin{split}
    \hat{\textbf{x}} = \arg\min_{\textbf{x}} \frac{1}{2}\sum_{i}||\textbf{y}_{i}-\mathcal{M}\odot\mathscr{F}S_{i}\textbf{x}||^{2}_{2} = \arg\min_{\textbf{x}} ||\textbf{y}-A\textbf{x}||^{2}_{2}
\end{split}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Sec 1.1. The prior} \textit{\dots  A regularizer expresses some prior\dots}\\
\response We were motivated by the formulation of \citep{fessler2010model, narnhofer2021bayesian, BayesianDeep}. 
But we totally agree to the point made by \rc\ and changed the text accordingly. 
Please find the following line in Sec. 1.1 footnote;\\
%\colorbox{blue!05}{
%$The  regularization  term, $R(\textbf{x})$,  has  a  %relation  with the  prior\dots
%}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 1.1. Vector in boldface} \textit{\dots please distinguish vectors from scalar values by e.g. making them bold or adding an arrow superscript\dots}\\
\response 
All the vectors are now in boldface font.
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 1.1. Tikonov Regularization} \textit{\dots The Tikhonov Regularizer is famous as a specific choice of one $R_i(x)$ and has a closed form solution \dots}\\
\response Agreed! 
Please see the following line in the main draft;\\
\colorbox{blue!05}{
However, the formulation in Eqn. \ref{eq_2_least_square} is under-determined if data is undersampled\dots
}
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 1.3. Kernels, non-uniform FFT} \textit{\dots Grappa-like methods are used in the multi-coil setting. In this setting the problem is usually not under-determined but over-determined. Also the kernels are just an analytical solution to this problem and no regularizer. This was shown due to its connection to SENSE}\\
\textit{\dots nuFFT just computes a FFT from non-uniformly sampled data which has nothing to do with multiple coils\dots}\\
\response Thanks for the comment! 
We have modified that paragraph. 
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 2. Weighted Sum} \textit{In a multicoil (say N coils) measurement we get measurements of multiple coils $y_i$ (of dimension $D$) which can then be assembled in some total vector of measurements by concatenating them to give a $N*D$ measurement vector. I don't understand why this weighted sum is formed here. It's surely not a good model of the measurement process. I believe it's an artifact of how the SMASH method is derived which actually puts the data in this form. But in that case the text needs to explain this much clearer.}\\
\response Sorry for the inconvenience! 
The discussion of equation $\mathcal{M}\odot\mathscr{F}S_{i}\textbf{x} + \eta$ is moved to Sec. \ref{sec_classical_k_space_methods} in the discourse of SMASH methodology. 
Please see the following line (font color: blue) in Sec. \ref{sec_classical_k_space_methods};\\
\colorbox{blue!05}{
So, in SMASH a k-space measurement $\textbf{x}$, also known as a composite signal \dots
}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 2.2. Eqn 14, 15} \textit{\dots why multply with an Identity matrix? By definition this should be an operation not changing anything\dots}\\
\response 
The $I$ is not the identity matrix but $I = S\textbf{x}$. 
In SENSE, a pixel location $(i,j)$ is a weighted sum of coil sensitivities, i.e.;
\begin{equation}
    I_{k}(i,j) = \sum_{k=1}^{N_c}\sum_{j=1}^{N_2} S_{kj}\textbf{x}(i,j),
    \label{eq_100000}
\end{equation}
where $N_{2}$ is the height of image $\textbf{x}\in R^{N_{1}\times N_{2}}$, $N_c$ is the number of coils, and $ S_{k}$ is the coil sensitivity of the $k^{th}$ coil. 
The $I_{k}$ is the k$^{th}$ coil image that has aliased pixels at a certain position, and $i$ is a particular row and $j=\{1, \cdots, N_2\}$ is the column index counting from the top of the image to the bottom. 
The $S$ is the sensitivity matrix that assembles the corresponding sensitivity values of the coils at the locations of the involved pixels in the full FOV image $\textbf{x}$. 
The coil images $I_{k}$, the sensitivity matrix $S$, and the image $\textbf{x}$ in Eqn. \ref{eq_100000} can be re-written as;
\begin{equation}
    I = S\textbf{x}.
\end{equation} 
We have modified the draft accordingly. 
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 2.2. Stochastic modelling} \textit{\dots I am unclear what this sentence wants to tell me. I am not aware about this stochastic modelling \dots Instead it operates on X-ray transformed images\dots}\\
\response 
By stochastic modeling, we mean to say a stochastic modeling framework that justifies the use of non-quadratic regularization functionals by tying them to some generative, continuous-domain signal model. 
Such approach builds upon the recent theory of sparse stochastic processes which are specified as solutions of stochastic differential equations (SDE) driven by non-Gaussian noise. 
We modified the draft and removed \citep{feldkamp1984practical}$^{'}$s citation as it does not fit the context. 
We, instead, discussed the paper ``Reconstruction of biomedical images and sparse stochastic modeling'' [\textcolor{red}{7}] to show the MRI reconstruction using stochastic modeling. 
We modified Sec. 2.2 
%(font color: blue), i.e;\\
%\colorbox{blue!05}{
%Different from Total Variation (TV) approaches the proposed %a stochastic modeling\dots
%}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 2.2. Function $\psi(\cdot)$} \textit{Those are not total variation - only one specific choice of this function is total variation.}\\
\response Agreed! 
The draft tried to introduce TV and then other variations of the so-called ``potential functions''. 
We have now changed the wordings of Sec 2.2. font color: magenta
%, i.e.;\\
%\colorbox{blue!05}{
%A potential function based regularization takes \dots
%}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 3.1. CNN formulation} \textit{\dots That is true, but it's not possible in the mathematical model of a CNN you gave in 26\dots}\\
\response We largely followed the convolution operation equation shown in \citep{liang2020deep}. 
We have now modified Sec. 3.1. Neocognitron or the Convolutional Neural Network (CNN) paragraph. 
%We have added the following lines \\
%\colorbox{blue!05}{
%We show a vanilla kernel operation in Eqn. \ref{eq_CNN}\dots
%}
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 3.3. Autoencoder formulation} \textit{\dots Not sure if it's correct but it's definitely way more complicated than necessary\dots}\\
\response Thanks for the suggestion! We changed Eqn. \ref{eq_autoencoder}.
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Sec 5.3. Near-optimal} \textit{optimal in what sense and how did they prove that optimality?\dots}\\
\response The term ``near-optimality'' is used in the AUTOMAP paper itself. 
The text from the AUTOMAP paper is as follows: \textit{Inspired by the perceptual learning archetype, we have developed a data-driven unified image reconstruction \dots that learns a near-optimal reconstruction \dots} \citep{Automap}. 
The AUTOMAP paper used the term to convey its outstanding performance with respect to the ground truth data.
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{CRNN misses minute anatomical details} \textit{\dots why such a specific limitation? Is it just blurring of the image or is the network doing something specific in the image content? If it's the former I would urge you to reformulate this \dots}\\
\response It's the second one. 
The Convolutional Neural Network (CNN) due to its design losses some minute details. 
The CRNN is a CNN with recurrence network that tends to lose finer details in deeper layers.
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Discussion section comment 1} \textit{\dots
I am not completely sure what you mean here? They surely must have trained on natural images which were forward transformed using the MRI acquisition operator to work? If that is the case, it's less surprising because e.g. learning the Fourier transform is accurately possible to the price of large amounts of memory.}\\
\response We agree with the statement that theoretically ``\dots learning the Fourier transform is accurately possible to the price of large amounts of memory\dots''. 
But, it might not be the case practically for a typical deep learning method. 
The problem is two fold. \\
\underline{First:} Despite having access to large databases such as fastMRI, most inverse mapping methods e.g.,  GrappaNet, VariationalNET, MODL, J-MODL are far from accurately learning the Fourier transform. \\ 
\underline{Second:} The problem is much worse when there is a domain shift, i.e. a model trained on Knee MRI data set fails to perform on Brain MRI testing data. 
Thus, learning of the Fourier transform accurately (for the case of highly under-sampled data) paying the price of large amounts of memory is still a challenging goal. 

The work of AUTOMAP can address both these points to a large extent and hence can be considered as a methodology that can generalize. 


%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Discussion section comment 2} \textit{\dots This might be difficult because not doing that means acquiring fully sampled data, which takes long and typically has other drawbacks e.g. increased motion artifacts\dots}\\
\response We would like to point out that, not doing ``accelerated MRI'' using GRAPPA-like methods while collecting raw measurements doesn't necessarily mean acquiring fully sampled k-space data. For instance, one could collect fastMRI type undersampled k-space data \citep{zbontar2018fastmri} without imposing GRAPPA reconstruction after acquisition which typically takes the same acquisition time as methods that use GRAPPA on the raw k-space. 

%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
\vspace{0.4cm}

\noindent\textbf{Other minor comments} \\
We have also addressed all other minor comments given below:\\
\underline{In Abstract}\\
1. \textit{\dots thousands of papers \dots}\\
\underline{In Sec. 1 first paragraph}\\
2. \textit{\dots damaging radiation}\\
\underline{In Sec. 1.1}\\
3. \textit{change $\eta$ to $\eta \sim \mathcal{N}(\bm{0}, \bm{\Sigma})$}\\
4. \textit{\dots vectors are in boldface font\dots}\\
5. \textit{change $E = \mathcal{M}\odot\mathcal{F}\mathcal{S}$ to $A = \mathcal{M}\odot\mathcal{F}\mathcal{S}$}\\
6. \textit{\dots has no unique solution}\\
7. \textit{\dots from ``optimized'' to ``designed''}\\
\underline{In Sec. 3.1. Transformer}\\
8. \textit{\dots That's an empirical observation but may not hold generally\dots}\\
\underline{In Sec. 3.3. Autoencoder}\\
9. \textit{\dots Eqn. 28}\\
\underline{In Sec. 5.1.}\\
10.\textit{\dots This method \textbf{showed showed} better performance \dots}\\
\underline{In Sec. 6}\\
11. \textit{\dots running into hundreds}\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage

\noindent{\Large \textbf{Rebuttal References}}\\
\begin{enumerate}
    \item Yamashita, R., Nishio, M., Do, R.K.G. et al. Convolutional neural networks: an overview and application in radiology. Insights Imaging 9, 611–629 (2018).
    \item H. K. Aggarwal, M. P. Mani and M. Jacob, "MoDL: Model-Based Deep Learning Architecture for Inverse Problems," in IEEE Transactions on Medical Imaging, vol. 38, no. 2, pp. 394-405, Feb. 2019, doi: 10.1109/TMI.2018.2865356.
    \item Recurrent Neural Networks, https://en.wikipedia.org/wiki/Recurrent\_neural\_network
    \item Raj, A., Bresler, Y. &amp; Li, B.. (2020). Improving Robustness of Deep-Learning-Based Image Reconstruction. Proceedings of the 37th International Conference on Machine Learning, in Proceedings of Machine Learning Research 119:7932-7942.
    \item Zhang, Jinwei, et al. “Fidelity imposed network edit (FINE) for solving ill-posed image reconstruction.” Neuroimage 211 (2020): 116579.
    \item Cheng, K., Calivá, F., Shah, R., Han, M., Majumdar, S. &amp; Pedoia, V.. (2020). Addressing The False Negative Problem of Deep Learning MRI Reconstruction Models by Adversarial Attacks and Robust Training. Proceedings of the Third Conference on Medical Imaging with Deep Learning, in Proceedings of Machine Learning Research, 121:121-135.
    \item Bostan, E., Kamilov, U., & Unser, M. (2012, May). Reconstruction of biomedical images and sparse stochastic modeling. In 2012 9th IEEE International Symposium on Biomedical Imaging (ISBI) (pp. 880-883). IEEE.
\end{enumerate}







